The Widespread Adoption of Large Language Model-Assisted Writing Across Society

The recent advances in large language models (LLMs) attracted significant public and policymaker interest in its adoption patterns. In this paper, we systematically analyze LLM-assisted writing across four domains-consumer complaints, corporate communications, job postings, and international organization press releases-from January 2022 to September 2024. Our dataset includes 687,241 consumer complaints, 537,413 corporate press releases, 304.3 million job postings, and 15,919 United Nations (UN) press releases. Using a robust population-level statistical framework, we find that LLM usage surged following the release of ChatGPT in November 2022. By late 2024, roughly 18% of financial consumer complaint text appears to be LLM-assisted, with adoption patterns spread broadly across regions and slightly higher in urban areas. For corporate press releases, up to 24% of the text is attributable to LLMs. In job postings, LLM-assisted writing accounts for just below 10% in small firms, and is even more common among younger firms. UN press releases also reflect this trend, with nearly 14% of content being generated or modified by LLMs. Although adoption climbed rapidly post-ChatGPT, growth appears to have stabilized by 2024, reflecting either saturation in LLM adoption or increasing subtlety of more advanced models. Our study shows the emergence of a new reality in which firms, consumers and even international organizations substantially rely on generative AI for communications.

==> FigurePlans.tex <==


Figure 1 (all domains): 
a, academic writing: (alpha value, arXiv abstract)
b, job posting
c, media: press release
d, (patent) < 10\%
======


Figure 1B (all domains): 
a, word frequency, academic writing
b, media: press release
c, job posting



Figure 2 (domain 1: academic writing): 
- Same as Figure 4 \textbf{Associations between LLM-modification and scientific publishing characteristics in \textit{arXiv} computer science papers. } 
- and Figure 5, \textbf{Regional trends in the adoption of large language models (LLMs) for academic writing.}  
    - arXiv probably not extending 
    - extend bioRxiv 


Figure 3 (domain 2: job posting): 
a, --- cut by the number of employees / or other metrics, rather than median number of job post.  
- direct on small firms. 
- direct on young firms. 
- direct on grow firms. 
b, 
c, 
d, year. 

Send Weixin job posting examples. 





Figure 4 (domain 2: media: press release): 
a, different categories. 
b, 
c, 
d, 





